Safest Nearby Neighbor Queries in Road Networks (Full Version)

Traditional route planning and k nearest neighbors queries only consider distance or travel time and ignore road safety altogether. However, many travellers prefer to avoid risky or unpleasant road conditions such as roads with high crime rates (e.g., robberies, kidnapping, riots etc.) and bumpy roads. To facilitate safe travel, we introduce a novel query for road networks called the k safest nearby neighbors (kSNN) query. Given a query location $v_l$, a distance constraint $d_c$ and a point of interest $p_i$, we define the safest path from $v_l$ to $p_i$ as the path with the highest path safety score among all the paths from $v_l$ to $p_i$ with length less than $d_c$. The path safety score is computed considering the road safety of each road segment on the path. Given a query location $v_l$, a distance constraint $d_c$ and a set of POIs P, a kSNN query returns k POIs with the k highest path safety scores in P along with their respective safest paths from the query location. We develop two novel indexing structures called Ct-tree and a safety score based Voronoi diagram (SNVD). We propose two efficient query processing algorithms each exploiting one of the proposed indexes to effectively refine the search space using the properties of the index. Our extensive experimental study on real datasets demonstrates that our solution is on average an order of magnitude faster than the baselines.

==> sections/1_Abstract.tex <==
\begin{abstract}
\revised{Safety on the roads has become a major concern in recent days. Travellers prefer to avoid road inconveniences that may occur from crime incidents, street harassment, protests or riots during unrest in a country. To facilitate safe travel, }we introduce a novel query for road networks called the $k$ safest nearby neighbor (SNN) query. Given a query location $v_l$, a distance constraint $d_c$ and a point of interest $p_i$, we define the safest path from $v_l$ to $p_i$ as the path with the highest \emph{path safety score} among all the paths from $v_l$ to $p_i$ with length less than $d_c$. The path safety score is computed considering the road safety of each road segment on the path. Given a query location $v_l$, a distance constraint $d_c$ and a set of POIs $P$, a $k$SNN query returns $k$ POIs with the $k$ highest path safety scores in $P$ along with their respective safest paths from the query location. We develop two novel indexing structures called $Ct$-tree and a safety score based Voronoi diagram (SNVD). We propose two efficient query processing algorithms each exploiting one of the proposed indexes to effectively refine the search space using the properties of the index. Our extensive experimental study on real datasets demonstrates that our solution is on average an order of magnitude faster than the baseline.
\end{abstract}

==> sections/temp.tex <==

\textbf{\emph{Pruning Effectiveness:}} 
In this set of experiments, we investigate the effectiveness of our pruning rules for the search space refinement.  \changed{Table~\ref{Table:Pruning} 
summarizes the experiment results in the default setting of the parameters in terms of the query processing time, number of network vertices accessed $|V_a|$ and number of valid paths explored in road networks for different approaches when different pruning rules are applied. The Basic  Algorithm includes only Pruning Rule~\ref{lemma:pruning1} (i.e., considers only valid paths).} The performance of our algorithms are the best when all pruning rules are applied, which in turn means that each of the pruning rule contributes in improving the efficiency of our algorithms.
\ifTKDE
\changed{Table~\ref{Table:Pruning}  also explains why SNVD is faster than $Ct$-tree and $Ct$-tree is faster than INE based approach.}
\else
\changed{Table~\ref{Table:Pruning} also shows why SNVD outperforms the other two algorithms. Note that the number of valid paths explored by the Basic Algorithm corresponds to $n_p$, $n^\prime_p$ and $n^{\prime\prime}_p$ in the complexity analyses of INE, $Ct$-tree and SNVD, respectively. Applying all pruning rules reduces the number of paths explored -- the percentage values w.r.t. the Basic Algorithm are shown in parentheses. These percentage values can be used to obtain effect factors $r$, $r^\prime$ and $r^{\prime\prime}$ in the complexity analyses (e.g., $50\%$ reduction in number of paths implies that the effect factor is $100/50=2$). Generally, $n^{\prime\prime}_p > n^\prime_p > n_p$ and $r^{\prime\prime} > r^{\prime} > r$ which explains why SNVD is faster than $Ct$-tree and $Ct$-tree is faster than INE based approach. }


\ifTKDE
\input{sections/table4_short}
\input{sections/table5_short}
\else
\input{sections/table4_long}
\input{sections/table5_long}






